Sonic: Fast and Transferable Data Poisoning on Clustering Algorithms

Data poisoning attacks on clustering algorithms have received limited attention, with existing methods struggling to scale efficiently as dataset sizes and feature counts increase. These attacks typically require re-clustering the entire dataset multiple times to generate predictions and assess the attacker's objectives, significantly hindering their scalability. This paper addresses these limitations by proposing Sonic, a novel genetic data poisoning attack that leverages incremental and scalable clustering algorithms, e.g., FISHDBC, as surrogates to accelerate poisoning attacks against graph-based and density-based clustering methods, such as HDBSCAN. We empirically demonstrate the effectiveness and efficiency of Sonic in poisoning the target clustering algorithms. We then conduct a comprehensive analysis of the factors affecting the scalability and transferability of poisoning attacks against clustering algorithms, and we conclude by examining the robustness of hyperparameters in our attack strategy Sonic.

==> sections/00_skeleton.tex <==
\newpage
\section{Skeleton}

\subsection{Introduction}

\begin{enumerate}

    \item Overview of the importance of clustering algorithms in various domains;
    \item Simple explanation on incremental clustering algorithms;
    \item Discussion on the feasibility of attacks to clustering in not toy scenarios;
    \item Objectives and contributions of your research.
    
\end{enumerate}

\subsection{Methodology}
\begin{enumerate}

    \item Structure of the genetic poisoning attack;
    \item Framework to exploit the advantage of incremental clustering algorithms.
    
\end{enumerate}

\subsection{Experimental setup}
\begin{enumerate}

    \item Detail the datasets used for evaluation, including their characteristics and sources.
    \item Outline the parameters and metrics used to evaluate the performance of clustering algorithms.
    \item Describe which experiment have been done (ablation, time, main, ecc...)

    
\end{enumerate}

\subsection{Experimental results}
\begin{enumerate}
    \item divide the section in the different experiments done and present them
    \item Provide quantitative and qualitative analyses of the performance of hierarchical clustering algorithms under each experiment section
    \item Include visualizations and comparisons to illustrate the impact of the proposed approach.
\end{enumerate}

\subsection{Related Work}
\begin{enumerate}
    \item Review existing literature on adversarial data poisoning in clustering algorithms.
    \item Discuss previous research efforts to address vulnerabilities in hierarchical clustering algorithms and their limitations. (If any)
    \item Highlight any relevant studies on incremental clustering algorithms and their applications in adversarial settings. (if any)
\end{enumerate}

\subsection{Conclusions and future works}
\begin{enumerate}
    \item Summarize the key findings and contributions.
    \item Discuss the implications of the results for the security and robustness of clustering algorithms.
    \item Suggest potential avenues for future research, such as exploring alternative attack strategies or refining the proposed approach.
\end{enumerate}
